Advancing Mathematical Reasoning in Language Models: The Impact of Problem-Solving Data, Data Synthesis Methods, and Training Stages

Mathematical reasoning remains a challenging area for large language models (LLMs), prompting the development of math-specific LLMs such as LLEMMA, DeepSeekMath, and Qwen2-Math, among others. These models typically follow a two-stage training paradigm: pre-training with math-related corpora and post-training with problem datasets for supervised fine-tuning (SFT). Despite these efforts, the improvements in mathematical reasoning achieved through continued pre-training (CPT) are often less significant compared to those obtained via SFT. This study addresses this discrepancy by exploring alternative strategies during the pre-training phase, focusing on the use of problem-solving data over general mathematical corpora. We investigate three primary research questions: (1) Can problem-solving data enhance the model's mathematical reasoning capabilities more effectively than general mathematical corpora during CPT? (2) Are synthetic data from the same source equally effective, and which synthesis methods are most efficient? (3) How do the capabilities developed from the same problem-solving data differ between the CPT and SFT stages, and what factors contribute to these differences? Our findings indicate that problem-solving data significantly enhances the model's mathematical capabilities compared to general mathematical corpora. We also identify effective data synthesis methods, demonstrating that the tutorship amplification synthesis method achieves the best performance. Furthermore, while SFT facilitates instruction-following abilities, it underperforms compared to CPT with the same data, which can be partially attributed to its poor learning capacity for more challenging problem-solving data. These insights provide valuable guidance for optimizing the mathematical reasoning capabilities of LLMs, culminating in our development of a powerful mathematical base model called MathGPT-8B.

==> Tables/data_composition.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table}[]
\caption{Distribution of dataset for each groups.}
\begin{tabular}{|l|llll|l|llll|l}
\cline{1-10}
        & \multicolumn{4}{c|}{General Corpus}                                                                                                           & \multicolumn{1}{c|}{Mathematical Corpus} & \multicolumn{4}{c|}{Problem-solving Data}                                                                            &  \\ \cline{1-10}
Dataset & \multicolumn{1}{l|}{{\ul Arxiv}} & \multicolumn{1}{l|}{{\ul AlgebraicStack}} & \multicolumn{1}{l|}{{\ul StarCoder}} & {\ul General Knowledge} & {\ul OpenWebMath}                        & \multicolumn{1}{l|}{{\ul NuminaMath}} & \multicolumn{1}{l|}{{\ul Lila}} & \multicolumn{1}{l|}{Seed} & Seed-Synthesis &  \\ \cline{1-10}
Tokens  & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{0}                    & \multicolumn{1}{l|}{0}               & 0                       & 0                                        & \multicolumn{1}{l|}{0}                & \multicolumn{1}{l|}{0}          & \multicolumn{1}{l|}{0}    & 0              &  \\ \cline{1-10}
\end{tabular}
\end{table}
